Attractor Basins in Concurrent Systems

A crucial question in analyzing a concurrent system is to determine its long-run behaviour, and in particular, whether there are irreversible choices in its evolution, leading into parts of the reachability space from which there is no return to other parts. Casting this problem in the unifying framework of safe Petri nets, our previous work has provided techniques for identifying attractors, i.e. terminal strongly connected components of the reachability space. What we aim at is to determine the attraction basins associated to those attractors; that is, those states from where all infinite runs are doomed to end in the given attractor, as opposed to those that are free to evolve differently. Here, we provide a solution for the case of safe Petri nets. Our algorithm uses net unfoldings and provides a map of all of those configurations (concurrent executions of the system) that lead onto cliff-edges, i.e. any maximal extension for those configurations lies in some basin that is considered fatal.

==> PiOne.tex <==

\begin{theorem}
\label{th:PiOneSuffices}
Let $\markn\in\reach(\markn_0)$, and set $\configs_\markn\define\{\confign\in\configs(\Pi_0(\markn_0):~\marking{\confign}=\markn)\}$. For every $\confign\in\confign_\markn$, let $\Pi_\confign$ be the prefix obtained by appending  a copy of $\Pi_0(\markn)$ after $\confign_\markn$, and let $\Pi_\confign^* \define\Pi_\confign\cap\Pi_1(\markn_0)$.
Then for any $\hat{\confign}\in\configs_\markn$, one has 
\begin{eqnarray}
\label{eq:PiOne}
\Pi_{\hat{\confign}}&=&\bigcup_{\confign\in\configs_\markn}\isom_{(\confign,\hat{\confign})}\left(\Pi_\confign^*\right).
\end{eqnarray}
\end{theorem}
\bepr
Fix $\markn$ and $\confign_\markn$. 
(compare Prop. 4.9. in~\cite{ERV02}) Let $\confign_1$ be a configuration such that $\confign\subsetneq\confign_1$ and $\marking{\confign_1}=\markn$. If $\confign_1$ is not a configuration of $\Pi_1(\markn_0)$, then it must contain a cutoff-1 event $e$ and decompose as $\confign_1=\cone{e}\oplus E_1$ for some event set $E_1$. By the choice of $e$, there must exist some cutoff-0 event $e'$ such that $\cone{e'}$ 
\eepr




We have the following two easy properties, which are  useful for future reference.
\begin{lem}\label{le:free}
\begin{enumerate}
    \item Let $\tup{\markn_1,\ldots,\markn_n}$ be a reachability cycle. Then either $\markn_i$ is doomed for all $i=1,\ldots,n$, or $\markn_i$ is free for all $i=1,\ldots,n$.
\item
A reachable marking $\markn$ of $\netn=\tup{\onlynetn,\markn_0}$ is free iff there exist a  reachability cycle $\tup{\markn_1,\ldots,\markn_n}$ such that $\markn\move{*}\markn_1$ and
 $\markn_1\not\in\badstates$.
 \end{enumerate}
\end{lem}

\subsection{\textsc{FreeCheck} using $\Pi_0$  and a little more}

Complementing the general algorithm \textsc{MinDoo}, we now present a method for finding all minimally doomed markings on a fixed, finite prefix.
% $\Pi_\viables$.
%; this $\Pi_\viables$ is constructed as a prefix of $\Pi$, and is in general a proper prefix. 
As above, fix a safe Petri net $\netn_0=\tup{\place,\trans,\flow,\markn_0}$ and a set $\badstates\subseteq 2^\place$ of bad markings.

Compute the first complete prefix $\Pi_0(\onlynetn,\markn_0)=\tup{\oplace^0,\otrans^0,\oflow^0,\cutn_0}$,
% of $\netn_0$, 
and let
    \begin{eqnarray*}
   \configs_0&\define&\confoff(\Pi_0)
   %\max\left(\configs\left(\prefixn_0\right)\right)\backslash \badconfs
   \\
   \mathcal{M}_{\configs_0}&\define& \marking{\configs_0}
   %\left\{\right\}
    \end{eqnarray*}
    be, respectively, the set of cutoff configurations of $\Pi_0$, and of those cutoff markings  that are not bad. If at this stage one detects that $\markings_?=\emptyset$, the construction can stop  here since no free state is reachable.
   % Indeed, if any $\markn\in\badstates$ is reachable, then at least one configuration in $\max(\configs(\prefixn_0))$ must lie in $\badconfs$ since $\Pi_0$ is complete and $\badstates$ is absorbing. 

Now, set $\overline{\markings}_\viables\define\emptyset$,\fxnote{What does $\overline{\markings}_\viables$ describe?} let $\mathcal{G}_?=(\{1,\ldots,k\},\emptyset)$\fxnote{ Do you mean $\{\markn_1,\ldots,\markn_k\}$? }  be the disconnected directed graph over $\markings_?$, and let wlog $\markings_?=\{1,\ldots,k\}$; we perform for each $i\in\{1,\ldots,n\}$ a  reachability test,
using a complete prefix $\Pi(i)$ of $\tup{\onlynetn,\markn_i}$. The test checks whether an instance of any marking in $\{\markn_0\}\cup\markings_?$ is reachable from $\markn_i$; depending on the outcome of this test, we have one of the following cases: 
\begin{itemize}
    \item $\markn_0$ or $\markn_i$ is reachable from $\markn_i$; in this case, one obviously has a non-bad cycle reachable from $\markn_i$ and thus from $\markn_0$, and we
    add $\markn_0$ (if necessary) and $\markn_i$ to $\overline{\markings}_\viables$.
    \item Some marking $\markn_j\not \in \{\markn_0,\markn_i\}$ such that $\markn_j\in\overline{\markings}_\viables$ is  reachable from $\markn_i$: add $\markn_i$ to $\overline{\markings}_\viables$.
    \item Neither of the above holds, but some $\markn_j\in\markings_?\backslash\{\markn_i\}$ is  reachable from $\markn_i$: add an arc from $i$ to $j$ to $\mathcal{G}$.
\end{itemize}

When all $i$ have been inspected, propagate the doomed and free conditions along $\mathcal{G}$:
\begin{itemize}
    \item Markings from which a free one is reachable, are themselves free: $\viables_!\define\{\markn\in\markings_!:~\markn\to^*{\markings}_\viables~ \mathit{in}~\mathcal{G}\}$ \fxnote{Is $\markings_?=\markings_!$ ?}
    \item All bad markings are doomed, and so are those that are reachable from a doomed marking: $\doomarks_!\define\badstates\cup\{\markn\in\markings_!:~\badstates\to^*\markn~ \mathit{in}~\mathcal{G}\}$.
\end{itemize}
Once  the status  (doomed vs free) of all configurations in $\confoff$ has been decided, one determines the status of an arbitrary reachable marking $\markn$ as follows:
\begin{itemize}
    \item Compute the set $\configs_0^\markn\define\{\confign\in\configs (\Pi_0):~\marking{\confign}=\markn\}$ (note that $\configs_0^\markn$ cannot be empty, because of completeness of $\Pi_0$);
    \item for every $\confign\in\configs_0^\markn$, let $\confoff^\confign\define\{\hat{\confign}\in\confoff:~\confign\subseteq\hat\confign\}$.
    \item Inspect the marking set 
    $\markings_!^\markn\define\bigcup_{\confign\in\configs_0^\markn}\confoff^\confign\subseteq\markings_!$; iff any $\markn_!\in\markings_!^\markn$ is free, then so is $\markn$, otherwise $\markn$ is doomed.
\end{itemize}
Let \textsc{FreeCheck}$(\markn)$ be the boolean predicate that is \textsc{true} iff $\markn$ is free, and \textsc{false} otherwise, i.e. iff $\markn$ is doomed, computed by the above algorithm.\fxnote{ Do we have to prove that the algo works?}

\textbf{NOTE :}{ all this would be better written in pseudocode ... }

==> freecheck.tex <==
\subsection{Algorithm \textsc{FreeCheck}}
\begin{algorithm}[hbt!]
\caption{Algorithm \textsc{FreeCheck}}\label{alg:two}
\KwData{Safe Petri Net $\petrinet=\tup{\place,\trans,\flow,\markn}$ and $\badstates\subseteq 2^{\place}$}
\KwResult{\textsc{True} if $\markn$ is free, \textsc{False} otherwise}
$\mindooout\gets\emptyset$;~
$\worklist \gets \emptyset$\;
\ForEach{$\confign\in\min_{\subseteq}(\badconfs^0)$}{
    $\confign'\gets\shaved{\confign}$\;
    $\worklist\gets\worklist\cup\{\confign'\}$\;
}
\While{$\worklist\neq\emptyset$}{
    Pick $\confign\in\worklist$;
    $\addit\gets \true$\;
    \uIf{NOT \textsc{FreeCheck}$(\marking{\confign\backslash\crest{\confign}})$}{
            $\addit\gets \false$\;
           $\confign'\gets\shaved{\confign\backslash\crest{\confign}}$\;
            $\worklist \gets (\worklist\cup\{\confign'\})$\;
            }
    \Else{
        \ForEach{$\otransn\in\crest{\confign}$}{
            \If{NOT \textsc{FreeCheck}$(\marking{(\confign\backslash\{\otransn\})}$}{
                $\addit\gets \false$\;
                $\confign'\gets\shaved{\confign\backslash\{\otransn\}}$\;
                $\worklist \gets \worklist\cup\{\confign'\}$\;
            }
    }}
    $\worklist\gets\worklist\backslash\{\confign\}$\;
    \If{$\addit$}{
        $\mindooout\gets\mindooout\cup\{\confign\}$\;
      }}
\Return{$\mindooout$}
\end{algorithm}


==> freerubbish.tex <==
\fxnote{From now on, need to rethink}
\begin{theorem}
For $\markn\in\markings_?$, $\markn$ is free iff $\markn\in\markings_!\overline{\markings}_\viables\cup\{\markn_j:~j\in\mathcal{I}_!\}$
\end{theorem}
\fxnote{not finished}
\bepr By construction of $\markings_!$, all its members are free by lemma~\ref{le:free}; assume now that $\markn$ is free.
By completeness, there must exist some configuration $\confign_\markn$ of $\Pi_0$ such that $\marking{\confign_\markn}=\markn$. Since $\markn$ is assumed free, there is at least one configuration $\confign\in\max(\configs(\Pi_0))$
such that $\confign_\markn\subseteq\confign$ and $\confign\not\in\badconfs$; denote the set of these $\Pi_0$-maximal configurations by $\configs_\markn$, and the set of their markings by $\markings_\markn$. If some marking in $\markings_\markn$ does not allow to reach any cycle for non-bad markings, $\markn$ is doomed, contradicting our assumption. Hence there must be some path $\markn\markn^0\ldots\markn^m\markn_1$ to a cycle marking $\markn_1$ in the notation of Lemma~\ref{le:free}. Clearly, there must exist $\nu\in\{1,\ldots,m\}$ such that that $\markn^\nu$ is an end marking of $\pi_\markn$ and thus $\markn^\nu\in\markings_?$, hence we have a path ...
\eepr


In $\Pi_1$, mark all bad end markings and all non-bad, but (according to Theorem~\ref{th:freetest}) non-free end markings as \emph{doomed}; then, proceed by shaving and rubbing to identify the minimally doomed configurations contained in $\Pi_1$.
Let $\tup{\markn_1,\ldots,\markn_n}$ be a reachability cycle of $\netn$

Denote by $\rabbit_0\define\marking{\max(\configs(\Pi_0))}$ the set of $\Pi_0$'s end markings. Let $\cycle\define\tup{\markn_1,\ldots,\markn_n}$ be a reachability cycle of $\netn$. By completeness, we know that all markings in $\cycle$ must be represented in $\Pi_0$. Conversely, there
must exist at least one marking $\markn_\cycle$ in $\rabbit_0$ such that $\markn_1$ (and thus every $\markn_i$ in $\cycle$) is reachable from $\markn_\cycle$.

==> game.tex <==
\section{How to Win a Survival Game}
\label{sec:game}
The results from the previous section give indications on how one should play a 'survival game' in which a supervisory player blocks certain transitions in order to avoid doom and keep the system viable. 
\subsection{Formalization of the Survival Game}
Assume a player $\player$ (e.g. a park ranger) strives to avoid doom for the ecosystem under their supervision, and to keep the system viable against adversities which we model as the choices of an adversarial environment player $\enviro$. 
The possible actions of $\player$ are described by a set of transitions $\trans_\player\subseteq\trans$, which $\player$ is capable of \emph{blocking}. All uncontrolled transitions can be selected freely by $\enviro$.   
Assuming the individual transitions in the system's evolution are sufficiently slow, we may imagine that $\enviro$ and $\player$ take turns in the game; $\enviro$ makes the system evolve, using both uncontrolled transitions from $\trans\backslash\trans_\player$ and controlled transitions from $\trans_\player$ that $\player$ has chosen not to block. This evolution takes the system into a new configuration $\confign$ which $\player$ observes; $\player$ chooses a set $\block\subseteq\trans_\player$ and blocks all $\transn\in\block$, to which $\enviro$ reacts using transitions from $\trans\backslash\block$, and so forth. 

That is, the player $\player$ is characterized by a function
\begin{eqnarray}
\block:\finfigs(\petrinet)&\to&2^{\trans_\player}\\
\confign&\mapsto&\block\define\block(\confign),
\end{eqnarray}
whereupon $\player$ transmits the set $\choice\define\block(\confign)$ to $\enviro$, etc. A \emph{play} of this game is thus a configuration 
\begin{eqnarray}
\confign&=& \confign_1\concat\confign_2\concat\ldots\concat\confign_n,
\end{eqnarray}
where, with $\consum_i\define\konkat_{j=1}^i\confign_j$, one has for all $i\in\{1,\ldots,n\}$
\begin{enumerate}
  \item     
 $\confign_i\in\finfigs_{\choice_i}(\petrinet_{\consum_{i-1}})$ and 
  \item $\choice_i=\block(\consum_{i-1})$.
\end{enumerate}
$\enviro$ wins in every play $\confign$ such that $\confign\in\doofigs$; $\player$ wins if they can prevent $\enviro$ from winning in every circumstance.
$\player $ wins in every infinite play $\confign\in\viables$; otherwise, $\enviro$ wins.
\subsection{$\player$ wins with a sentinel on every ridge}
In view of the above, let us call $\petrinet$ \emph{sustainable} iff for all ridges $\ridge$, $\player_\trans\cap\ridge\neq\emptyset$.  For $\petrinet$ sustainable, call a  a strategy $\block$
\emph{admissible} iff for all $\confign\in\finfigs(\petrinet)$, $\block(\confign)$
\begin{lemma}
If $\markn_0\not\in\doomarks$ and for every ridge $\ridge$ of $\petrinet$ one has \label{le:doomavoid} ,  then $\player$ can keep $\petrinet$ in the set of viable states.
 \end{lemma}
% To prepare the proof, let us introduce an auxiliary notion.
% \begin{definition}
% A viable configuration $\confign\in\viables$ is called \emph{dangerous} iff there exists a doomed configuration $\confign'\in\doofigs$ such that
% \begin{enumerate}
%     \item $\confign\subseteq\confign'$
%     \item $\crest{\confign'}\cap{\confign}\ne\emptyset$.
% \end{enumerate}
% \end{definition}
\bepr
It suffices to define $\block$ in such a way that all choices $\block(\confign)$ for $\confign\in\finfigs(\net,\markn_0)$ contain one transition in every ridge.
\eepr
That is, under the condition \emph{one sentinel on every ridge}, $\player$ is assured to win, even with a deterministic strategy that sets $\block\equiv(\trans_\player\cap\bigcup\ridge)$, where the union is taken over all ridges of $\petrinet$.

Another question is whether one can find a winning strategy $\block$ that is also \emph{maximally permissive} in the sense that every \emph{viable} marking remains reachable under $\player$'s moves.



==> junk.tex <==
To see this, we will proceed through several steps:
\begin{enumerate}
    \item For any initial marking $\markn_0$, $\Pi_0'(\markn_0)$ (and a fortiori $\Pi_0(\markn_0)$) contains all markings reachable from $\markn_0$~(\cite{ERV02}); in particular, $\Pi_0(\markn_0)$ contains a second instance of $\markn_0$ (the first being the initial cut of $\Pi_0(\markn_0)$) if and only if there is a non-empty loop sequence $\sigma$ satisfying $\markn_0$. 
    %Indeed, let $\sigma$
    \item For any $\markn$ reachable from $\markn_0$, $\Pi_0(\markn_0)$ contains at least one instance of $\markn$, i.e. a configuration $\confign_\markn$ such that $\marking{\confign_\markn}=\markn$. The freedom check for $\markn_0$ is therefore possible on any unfolding prefix that contains, for every reachable marking $\markn$ allowing a loop, a configuration on which this loop is performed.
    Lemma~\ref{le:PiOneSuffices} below will prove that $\Pi_1(\markn_0)$ is sufficient for this, completing the proof  of the claim.
\end{enumerate}
\begin{Lemma}
\label{le:PiOneSuffices} Let $\markn\in\reach(\markn_0)$ enable a non-empty firing sequence $\sigma$ such that $\markn\move{\sigma}\markn$. Then $\Pi_1(\markn_0)$ contains  configuration $\confign_1$ and $\confign_2$ such that 
\begin{enumerate}
    \item $\marking{\confign_1}=\marking{\confign_2}=\markn$ and
    \item % $\confign_2$ such that $\markn$ and 
    $\confign_1\subsetneq\confign_2$.
\end{enumerate}
\end{Lemma}
\bepr 
We actually show a stronger result (proof sketch):By completeness of $\Pi_0'(\markn_0)$, there exists $\confign_\markn\in\configs(\Pi_0(\markn_0))$ such that $\marking{\confign_\markn}=\markn$.Define $\Pi_\markn$ as the concatenation of $\confign_\markn\in\configs(\Pi_0)$ and its suffix in $\Pi_1$. Then, the McMillan prefix $\Pi^{McM}_0(\markn)$ of $\markn$ is contained in $\Pi_\markn$. Indeed, all events on the branches that extend $\confign_\markn$ and that are cutoff-1 for $\Pi_1(\markn_0)$ are also cutoff for $\Pi^{McM}_0(\markn)$ modulo isomorphism; but since the  mirror events for cutoffs in $\Pi^{McM}_0(\markn)$ may lie inside $\Pi_0$, some events may become cutoff for $\Pi^{McM}_0(\markn)$ without being cutoff-1 in $\Pi_1(\markn_0)$. One concludes that $\Pi^{McM}_0(\markn)$  has at most the non-cutoff events of $\Pi_1(\markn_0)$. Therefore, the loop $\markn\to\markn$ is represented in $\Pi_1$.
\eepr


==> oldalgo.tex <==

\fxnote{May not be needed anymore ...}

Start with the algorithm, make the theorem the correctness statement for the algo.
\begin{theorem}
A marking $\markn$ is free iff
\end{theorem}

\fxnote{The rest of this subsection can be simplified with the above.}
In a first step towards that, Theorem~\ref{th:notbad}  below uses a similar proof idea as Lemma 8 in~\cite{HRS-acsd13} in the context of fault  diagnosis.
Let us first recall the notion of \emph{spoilers}, introduced in  ~\cite{HRS-acsd13}:
\begin{definition}\textit{
A \emph{spoiler} of transition $\transn$ (or  event $\otransn$) is any $\transn'\in\trans$ ($\otransn'\in\otrans$) such that $\preset{\transn'}\cap\preset{\transn}\ne\emptyset$ ($\preset{\otransn}\cap\preset{\otransn'}\ne\emptyset$).
We write $\spoil{\transn}$  ($\spoil{\otransn}$) for the set of $\transn'$s ($\otransn$'s) spoilers.}
\end{definition}
Note that $\transn\in\spoil\transn$ for all $\transn\in\trans$. The spoilers of $\transn$ are characterized by the fact that their firing cancels any enabling of $\transn$; that is, by being either in conflict with $\transn$, or identical with $\transn$.
\begin{theorem}\label{th:notbad}{\it
A configuration $\confign\in\finfigs$ is \textbf{free} iff either a) there exists a finite maximal configuration $\confign'$ such that $\confign\subseteq\confign'\not\in\badconfs$, or b) there exist  configurations $\confign_1,\confign_2\in\finfigs$ such that 
\begin{enumerate}
    \item\label{con:nest} $\confign\subseteq\confign_1\subseteq \confign_2\notin\badconfs$;
    \item \label{con:mark}$\marking{\confign_1}=\marking{\confign_2}$;
    \item \label{con:spoil} for all events $\otransn\in\otrans$ such that $\confign_1\omove{\otransn}$, one has $\spoil{\otransn}\cap \confign_2\ne\emptyset$.
\end{enumerate}
}
\end{theorem}
Some comments are in order before giving the proof of Theorem~\ref{th:notbad}.
First of all, the requirement to check whether $\confign_2\not\in\badconfs$ can be met by checking whether $\marking{\confign_2}\in\clbadstates$.
Second, the spoiling condition (3) ensures that the process that takes $\confign_1$ to $\confign_2$ forms a loop whose iteration yields a run.

\bepr In the following, let $M:=\marking{C_1}$. We first prove the right-to-left implication. Case a) is obvious, so assume that b) holds.
Let $\confign_2=\confign_1\concat\hat{\confign}$; then by 2., we can append $\hat{\confign}$ to $\confign_2$, yielding a strictly increasing sequence of configurations $(\confign_n)_{n\in\NN}$
such that $\confign_{n+1}=\confign_n\concat \hat{\confign}$, and $\marking{\confign_n}=\markn$ for all $n$. By property~3, we know that $\hat{\confign}$ contains spoilers for all its initially enabled events , hence 
no transition remains enabled forever, and $\omega\define\bigcup_{n\in\NN}\confign_n$ is a maximal configuration. It remains to show that $\omega$ contains no bad configuration:
Suppose that there is $C'\subseteq\omega$ with $C'\in\badconfs$. Since $C'$ is finite, we have $C'\subseteq C_n$ for some $n$. But then, $M=\marking{C_n}$ is reachable from $\marking{C'}\in\badstates$,
contradicting our assumptions. Thus $\omega$ never enters a bad state, and $\confign$ is free. 


For the forward implication, assume that $\confign$ is free. Then there exists $\runn\in\runs_\confign$ such that $C'\notin\badconfs$ for all finite $C'\subseteq\runn$. If this $\runn$ can be chosen finite, then a) holds and we are done; so assume henceforth that $\runn$ must be chosen infinite. Clearly, there must exist a reachable marking $\markn$ that is visited an infinite number of times  by a family of  nested finite configurations $(\confign^n)_{n\in\NN}$ such that $\bigcup_{n\in\NN}\confign^n=\runn$. Let $\confign_1\define\confign^1$ and  $E':=\{\otransn:~\confign_1\omove{\otransn}\}$. Let $K$ be the smallest index such that for all $\otransn\in E'$, one has  $\spoil{\otransn}\cap\confign^K\ne\emptyset$; such a $K$ must exist since $\omega$ is maximal. Then $\confign_1$ and $\confign_2\define\confign^K$ have the required properties.
\eepr

Notice that the proof could be restructured by observing that case a) of Theorem~\ref{th:notbad} is indeed a special instance of case b). In fact, taking $\confign_1\define\confign_2\define\confign'$ with  $\confign'$ according to  case a), conditions 1 and 2 of part b) are obviously satisfied, and condition~3 holds vacuously since no event is enabled in $\confign_1=\confign'$.  We note in passeing that this observation is helpful in simplifying the implementation used for the experiments  below.

The interest of Theorem~\ref{th:notbad} lies in the following fact:
\begin{lemma}
\label{le:complix} For $\confign\in\finfigs$, checking whether $\confign$ is free can be done using finite prefix $\prefixn_1$ of $\unfolding(\net,\marking{\confign})$.
\end{lemma}
\bepr If $\confign$ is free, let $C_1$ and $C_2$ be the configurations witnessing this fact from Theorem~\ref{th:notbad}, and let $M:=\marking{C_1}=\marking{C_2}$. If such configurations exist, then $C_1$ can be chosen from the complete prefix $\prefixn_0$, and $C_2$ can be chosen from $\prefixn_1$, notably 
in the copy of  $\prefixn_{\marking{\confign_1}}$  appended after $\confign_1$. 

Checking whether the  configuration $\confign_2$ thus found is in $\badconfs$ is immediate, since it suffices to check whether its marking is in $\badstates$, using the fact that  $\badstates$ is reachability-closed. 
To check the spoiler condition (3) of Theorem~\ref{th:notbad}, it suffices to check whether the conditions of the cut of $\confign_1$ that are not consumed by $\confign_2$ enable some event.
\eepr


==> oldwreath.tex <==

, with the resulting configuration $\confign'$ still in $\badconfs$; this implies that despite the resolution of some conflicts after $\confign'$, the resulting branches \emph{all} lead to bad states. To detect such a situation, we explore the \emph{wreath} of shaved configuration $\confign$:
\begin{definition}{\it 
Let $\confign\in\finfigs$ such that $\shaved{\confign}=\confign$. The \emph{wreath} of $\confign$ is the set of configurations obtained by replacing a crest event of $\confign$ by one of its challengers:
\begin{eqnarray*}
\wreath{\confign}&\define&\left\{\confign_\otransn^{\otransn'}:~
\otransn\in\crest{\confign},~\otransn'\imcf\otransn
\right\},
\end{eqnarray*}
where $\confign_\otransn^{\otransn'}\define(\confign\backslash\{\otransn\})\cup\{\otransn'\}$.}
\end{definition}
 Partition $\wreath{\confign}$ into its doomed and viable parts, respectively, that is :
\begin{eqnarray*}
\doomed{\confign}&\define&\{\confign'\in \wreath{\confign}:~ \confign'~\mathit{is}~\mathit{doomed}\}\\
\viable{\confign}&\define&\{\confign'\in \wreath{\confign}:~ \confign'~\mathit{is}~\mathit{viable}\}
\end{eqnarray*}
It is easy to see that all $\confign_\otransn^{\otransn'}$ are indeed finite configurations.
We will give below an algorithm for identifying minimal doomed configurations; first, let us provide some further auxiliary notions.

   % \begin{itemize}
        \item Compute $\setn\define\wreath{\shaved{\confign}}$,\\
        $\doomed{\confign}$ and $\viable{\confign}$.
      %  \item \textsc{Forall} $\otransn\in\crest{\confign}$ \textsc{Do} 
     %   \begin{itemize}
      %      \item \textsc{Forall} $\otransn'\in\stern{\otransn}$ %\textsc
         
      %          \item Set  $\doomed_\otransn^{\otransn'}\define TRUE$ iff $\confign_\otransn^{\otransn'}$ is \emph{doomed}  
          %  \end{itemize}
          \item \textsc{If} $\doomed{\confign}=\emptyset$ 
            \begin{itemize}
            \item \textsc{Then} \begin{eqnarray*}
            \setn&\define&\setn\backslash\{\confign\}\\
            \mindofigs&\define&\mindofigs\cup \{\confign\}
            \end{eqnarray*}
            \item \textsc{else}
            \begin{eqnarray*}
            \confign'&\define&\bigcup_{\bar{\confign}\in\wreath{\confign}}\bar{\confign}\\
            \setn&\define&\left(\setn\backslash
            \left\{\confign\right\}\right)\cup\left\{\confign'\right\}
            \end{eqnarray*}
    \end{itemize}
   
\end{itemize}
\textsc{until} $\setn=\emptyset$
\end{itemize}
